Career Incentives, Risk-Taking, and Sorting Dynamics: Evidence from Top Financial Advisers

We examine how career concerns influence the behavior and mobility of financial advisers. Drawing on a uniquely comprehensive matched panel that combines employer-employee data with a longstanding national ranking, our study tests predictions from classic career concerns models and tournament theory. Our analysis shows that, in the early stages of their careers, advisers destined for top performance differ significantly from their peers. Specifically, before being ranked, these advisers are twice as likely to obtain a key investment license, experience customer disputes at rates up to seven times higher, and transition to firms with 80% larger total assets. Moreover, we find that top advisers mitigate the potential costs of their higher risk-taking by facing reduced labor market penalties following disciplinary actions. Leveraging exogenous variation from the staggered adoption of the Broker Protocol through an event-study framework, our results reveal dynamic sorting: firms attract high-performing advisers intensely within a short post-adoption period. These findings shed new light on the interplay between career incentives, risk-taking, and labor market outcomes in the financial services industry, with important implications for both firm performance and regulatory policy.

==> table/table_1_1.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize License: Series 65/66 (\%)}}                      \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&    43.37\sym{***}&    32.00\sym{***}&    18.98\sym{***}&    19.67\sym{***}&    21.92\sym{***}\\
                &   (3.28)         &   (2.72)         &   (2.07)         &   (2.16)         &   (2.42)         \\
\addlinespace
\specialcell{\scriptsize Top Adviser $\times$ After}&     5.82\sym{***}&     1.03         &    -5.06\sym{**} &    -4.12\sym{**} &    -6.11\sym{***}\\
                &   (1.92)         &   (1.88)         &   (2.09)         &   (1.98)         &   (1.73)         \\
\addlinespace
\specialcell{\scriptsize Series 63}&                  &   -22.93\sym{***}&   -17.13\sym{***}&                  &                  \\
                &                  &   (1.89)         &   (1.05)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Series 7}&                  &    44.43\sym{***}&    32.79\sym{***}&                  &                  \\
                &                  &   (1.85)         &   (1.16)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Series 6}&                  &    10.79\sym{***}&    -0.23         &                  &                  \\
                &                  &   (1.36)         &   (0.62)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Series 24}&                  &    -9.95\sym{***}&    -1.36\sym{**} &                  &                  \\
                &                  &   (2.12)         &   (0.63)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Experience}&                  &     0.62\sym{***}&     0.48\sym{***}&     0.84\sym{***}&                  \\
                &                  &   (0.15)         &   (0.08)         &   (0.09)         &                  \\
\addlinespace
\specialcell{\scriptsize Experience squared}&                  &    -0.00         &    -0.02\sym{***}&    -0.03\sym{***}&                  \\
                &                  &   (0.00)         &   (0.00)         &   (0.00)         &                  \\
\addlinespace
\specialcell{\scriptsize Tenure}&                  &    -4.04\sym{***}&    -7.27\sym{***}&    -6.13\sym{***}&    -4.67\sym{***}\\
                &                  &   (0.51)         &   (0.54)         &   (0.58)         &   (0.57)         \\
\addlinespace
\specialcell{\scriptsize Female}&                  &     0.02         &    -0.15         &    -0.17\sym{*}  &    -0.28\sym{***}\\
                &                  &   (0.16)         &   (0.10)         &   (0.09)         &   (0.10)         \\
\addlinespace
\specialcell{\scriptsize Number of Other Licenses}&                  &     3.80\sym{***}&     5.23\sym{***}&     4.22\sym{***}&     3.64\sym{***}\\
                &                  &   (0.68)         &   (0.29)         &   (0.31)         &   (0.51)         \\
\addlinespace
\specialcell{\scriptsize Cumulative Number of Switching Firms}&                  &     0.60\sym{**} &     1.53\sym{***}&     1.21\sym{***}&     0.99\sym{***}\\
                &                  &   (0.28)         &   (0.19)         &   (0.17)         &   (0.23)         \\
\addlinespace
\specialcell{\scriptsize Cumulative Number of Migration Across States}&                  &     3.65\sym{***}&     1.90\sym{***}&     1.84\sym{***}&     1.95\sym{***}\\
                &                  &   (0.48)         &   (0.19)         &   (0.17)         &   (0.21)         \\
\midrule
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&12,396,016         &12,396,016         &11,632,150         &10,614,118         &6,987,781         \\
\specialcell{\scriptsize \(R^2\)}&    0.003         &    0.217         &    0.472         &    0.554         &    0.649         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    35.96         &    35.96         &    36.02         &    34.98         &    30.88         \\


==> table/table_1_2_1.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Incidence of Customer Disputes (\%)}}             \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&     1.30\sym{***}&     1.01\sym{***}&     0.72\sym{***}&     0.60\sym{***}&     0.45\sym{***}\\
                &   (0.09)         &   (0.08)         &   (0.08)         &   (0.08)         &   (0.12)         \\
\addlinespace
\specialcell{\scriptsize Top Adviser $\times$ After}&    -0.32\sym{**} &    -0.40\sym{***}&    -0.00         &     0.10         &     0.27         \\
                &   (0.13)         &   (0.13)         &   (0.12)         &   (0.12)         &   (0.21)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&12,396,016         &12,396,016         &11,632,150         &10,230,894         &6,466,895         \\
\specialcell{\scriptsize \(R^2\)}&    0.000         &    0.003         &    0.085         &    0.158         &    0.286         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.36         &     0.36         &     0.36         &     0.34         &     0.29         \\


==> table/table_1_2_2.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Incidence of Customer Disputes (\%)}}             \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&     2.38\sym{***}&     2.02\sym{***}&     1.63\sym{***}&     1.49\sym{***}&     1.50\sym{***}\\
                &   (0.19)         &   (0.16)         &   (0.12)         &   (0.11)         &   (0.14)         \\
\addlinespace
\specialcell{\scriptsize Top Adviser $\times$ After}&    -1.31\sym{***}&    -1.35\sym{***}&    -0.77\sym{***}&    -0.63\sym{***}&    -0.70\sym{***}\\
                &   (0.22)         &   (0.23)         &   (0.15)         &   (0.13)         &   (0.14)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&12,396,016         &12,396,016         &11,632,150         &10,230,894         &6,466,895         \\
\specialcell{\scriptsize \(R^2\)}&    0.000         &    0.003         &    0.079         &    0.151         &    0.274         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.42         &     0.42         &     0.42         &     0.41         &     0.34         \\


==> table/table_2_1.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&    32.45\sym{***}&    27.31\sym{***}&    35.33\sym{***}&    24.72\sym{***}&    32.65\sym{***}&    21.97\sym{***}&    28.42\sym{***}&    21.56\sym{***}\\
                &   (3.78)         &   (3.90)         &   (3.20)         &   (3.82)         &   (3.29)         &   (3.50)         &   (2.78)         &   (2.42)         \\
\addlinespace
\specialcell{\scriptsize Series 63}&   -31.07\sym{***}&                  &   -29.71\sym{***}&                  &   -22.95\sym{***}&                  &    -9.69\sym{***}&                  \\
                &   (3.03)         &                  &   (1.94)         &                  &   (1.61)         &                  &   (1.42)         &                  \\
\addlinespace
\specialcell{\scriptsize Series 7}&    41.30\sym{***}&                  &    47.72\sym{***}&                  &    49.09\sym{***}&                  &    46.97\sym{***}&                  \\
                &   (2.30)         &                  &   (1.89)         &                  &   (1.92)         &                  &   (2.21)         &                  \\
\addlinespace
\specialcell{\scriptsize Series 6}&    12.17\sym{***}&                  &    14.43\sym{***}&                  &    12.84\sym{***}&                  &    10.65\sym{***}&                  \\
                &   (1.40)         &                  &   (1.69)         &                  &   (1.72)         &                  &   (1.78)         &                  \\
\addlinespace
\specialcell{\scriptsize Series 24}&    -9.64\sym{***}&                  &    -7.45\sym{***}&                  &    -9.85\sym{***}&                  &   -11.14\sym{***}&                  \\
                &   (1.98)         &                  &   (2.02)         &                  &   (2.27)         &                  &   (2.45)         &                  \\
\addlinespace
\specialcell{\scriptsize Experience}&     1.59\sym{***}&                  &     0.42\sym{***}&                  &     0.08         &                  &    -0.14         &                  \\
                &   (0.27)         &                  &   (0.15)         &                  &   (0.12)         &                  &   (0.10)         &                  \\
\addlinespace
\specialcell{\scriptsize Tenure}&    -4.62\sym{***}&    -3.39\sym{***}&    -4.99\sym{***}&    -4.93\sym{***}&    -4.40\sym{***}&    -5.97\sym{***}&    -3.29\sym{***}&    -6.34\sym{***}\\
                &   (0.55)         &   (0.54)         &   (0.59)         &   (0.63)         &   (0.65)         &   (0.73)         &   (0.58)         &   (0.86)         \\
\addlinespace
\specialcell{\scriptsize Female}&     0.97\sym{***}&    -0.45\sym{***}&     0.27         &    -0.55\sym{***}&     0.13         &    -0.33\sym{***}&    -0.03         &    -0.32\sym{***}\\
                &   (0.33)         &   (0.14)         &   (0.21)         &   (0.11)         &   (0.16)         &   (0.09)         &   (0.16)         &   (0.11)         \\
\addlinespace
\specialcell{\scriptsize Number of Other Licenses}&    -2.38         &     2.14\sym{**} &     0.43         &     2.66\sym{***}&     2.63\sym{***}&     3.32\sym{***}&     3.97\sym{***}&     4.12\sym{***}\\
                &   (1.53)         &   (0.86)         &   (0.87)         &   (0.66)         &   (0.76)         &   (0.53)         &   (0.70)         &   (0.45)         \\
\addlinespace
\specialcell{\scriptsize Cumulative Number of Switching Firms}&     6.75\sym{***}&     3.62\sym{***}&     3.72\sym{***}&     2.00\sym{***}&     1.60\sym{***}&     1.42\sym{***}&    -0.36         &     0.67\sym{***}\\
                &   (0.89)         &   (0.42)         &   (0.56)         &   (0.25)         &   (0.43)         &   (0.25)         &   (0.32)         &   (0.24)         \\
\addlinespace
\specialcell{\scriptsize Cumulative Number of Migration Across States}&     1.51\sym{*}  &     2.14\sym{***}&     2.48\sym{***}&     1.69\sym{***}&     3.41\sym{***}&     1.63\sym{***}&     4.63\sym{***}&     1.91\sym{***}\\
                &   (0.91)         &   (0.37)         &   (0.72)         &   (0.28)         &   (0.67)         &   (0.22)         &   (0.56)         &   (0.27)         \\
\midrule
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&3,657,615         &2,664,413         &2,606,353         &1,599,772         &2,035,744         &1,088,176         &1,629,282         &  783,964         \\
\specialcell{\scriptsize \(R^2\)}&    0.322         &    0.701         &    0.256         &    0.641         &    0.196         &    0.618         &    0.146         &    0.584         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    25.45         &    22.80         &    35.34         &    30.16         &    40.29         &    34.79         &    42.08         &    38.06         \\


==> table/table_2_2_1.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     0.35         &     0.35         &     1.12\sym{***}&     0.80\sym{**} &     1.08\sym{***}&     0.69\sym{**} &     1.09\sym{***}&     0.27\sym{*}  \\
                &   (0.25)         &   (0.37)         &   (0.24)         &   (0.32)         &   (0.24)         &   (0.35)         &   (0.13)         &   (0.16)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     0.09\sym{***}&     0.01         &     0.26\sym{***}&     0.26\sym{***}&     0.18\sym{***}&     0.22\sym{***}&    -0.07\sym{**} &     0.13\sym{***}\\
                &   (0.02)         &   (0.02)         &   (0.05)         &   (0.06)         &   (0.04)         &   (0.07)         &   (0.03)         &   (0.05)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&3,657,615         &2,573,792         &2,606,353         &1,499,646         &2,035,744         &  989,706         &1,629,282         &  694,692         \\
\specialcell{\scriptsize \(R^2\)}&    0.001         &    0.205         &    0.002         &    0.252         &    0.002         &    0.283         &    0.002         &    0.299         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.09         &     0.08         &     0.31         &     0.29         &     0.44         &     0.40         &     0.55         &     0.53         \\


==> table/table_2_2_2.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     0.74\sym{***}&     0.28         &     2.53\sym{***}&     2.36\sym{***}&     2.07\sym{***}&     1.51\sym{***}&     2.38\sym{***}&     1.79\sym{***}\\
                &   (0.22)         &   (0.22)         &   (0.37)         &   (0.41)         &   (0.23)         &   (0.24)         &   (0.27)         &   (0.28)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     0.15\sym{***}&     0.06\sym{**} &     0.41\sym{***}&     0.36\sym{***}&     0.19\sym{***}&     0.18\sym{***}&    -0.14\sym{***}&     0.15\sym{***}\\
                &   (0.03)         &   (0.02)         &   (0.08)         &   (0.10)         &   (0.05)         &   (0.06)         &   (0.05)         &   (0.06)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&3,657,615         &2,573,792         &2,606,353         &1,499,646         &2,035,744         &  989,706         &1,629,282         &  694,692         \\
\specialcell{\scriptsize \(R^2\)}&    0.001         &    0.199         &    0.003         &    0.243         &    0.002         &    0.277         &    0.002         &    0.289         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.12         &     0.11         &     0.42         &     0.38         &     0.54         &     0.48         &     0.64         &     0.60         \\


==> table/table_2_3_1.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     0.42\sym{**} &     0.60\sym{***}&     0.87\sym{***}&     0.81\sym{***}&     1.18\sym{***}&     0.97\sym{***}&     1.24\sym{***}&     0.96\sym{***}\\
                &   (0.18)         &   (0.11)         &   (0.13)         &   (0.10)         &   (0.11)         &   (0.11)         &   (0.11)         &   (0.11)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     1.02\sym{***}&     0.28\sym{***}&     0.88\sym{***}&    -0.03         &     0.82\sym{***}&    -0.01         &     0.82\sym{***}&     0.00         \\
                &   (0.13)         &   (0.07)         &   (0.09)         &   (0.04)         &   (0.11)         &   (0.05)         &   (0.15)         &   (0.05)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&3,657,615         &3,351,286         &2,606,353         &2,315,554         &2,035,744         &1,761,522         &1,629,282         &1,375,548         \\
\specialcell{\scriptsize \(R^2\)}&    0.109         &    0.366         &    0.107         &    0.337         &    0.111         &    0.327         &    0.121         &    0.337         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     7.87         &     7.89         &     7.73         &     7.74         &     7.65         &     7.67         &     7.57         &     7.58         \\


==> table/table_2_3_2.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     2.69\sym{***}&     2.40\sym{***}&     2.98\sym{***}&     2.38\sym{***}&     3.09\sym{***}&     2.47\sym{***}&     2.85\sym{***}&     2.27\sym{***}\\
                &   (0.33)         &   (0.34)         &   (0.27)         &   (0.30)         &   (0.29)         &   (0.34)         &   (0.28)         &   (0.31)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&    -0.22         &     0.09         &    -0.29         &     0.02         &    -0.09         &     0.12         &     0.10         &     0.08         \\
                &   (0.48)         &   (0.17)         &   (0.34)         &   (0.10)         &   (0.29)         &   (0.10)         &   (0.29)         &   (0.07)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&2,947,878         &2,692,018         &2,131,971         &1,882,487         &1,667,690         &1,430,944         &1,327,363         &1,107,899         \\
\specialcell{\scriptsize \(R^2\)}&    0.168         &    0.433         &    0.189         &    0.417         &    0.191         &    0.391         &    0.195         &    0.392         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    19.74         &    19.87         &    19.59         &    19.77         &    19.48         &    19.69         &    19.35         &    19.58         \\


==> table/table_2_4_1.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     0.55\sym{***}&     0.60\sym{***}&     1.09\sym{***}&     0.46\sym{***}&     1.24\sym{***}&     0.45\sym{***}&     1.19\sym{***}&     0.32\sym{***}\\
                &   (0.18)         &   (0.15)         &   (0.11)         &   (0.09)         &   (0.10)         &   (0.09)         &   (0.22)         &   (0.08)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     1.00\sym{***}&     0.35\sym{***}&     0.89\sym{***}&    -0.01         &     0.88\sym{***}&     0.01         &     0.66\sym{***}&     0.08\sym{**} \\
                &   (0.05)         &   (0.04)         &   (0.05)         &   (0.05)         &   (0.08)         &   (0.04)         &   (0.10)         &   (0.04)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Original Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&  348,579         &  194,079         &  261,402         &  113,945         &  182,486         &   61,069         &  134,185         &   38,527         \\
\specialcell{\scriptsize \(R^2\)}&    0.090         &    0.525         &    0.088         &    0.585         &    0.097         &    0.629         &    0.099         &    0.645         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     7.45         &     7.61         &     7.26         &     7.55         &     7.14         &     7.63         &     6.98         &     7.53         \\


==> table/table_2_4_2.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     2.52\sym{***}&     1.57\sym{***}&     3.23\sym{***}&     0.92\sym{***}&     3.04\sym{***}&     1.01\sym{***}&     2.64\sym{***}&     0.59\sym{***}\\
                &   (0.39)         &   (0.28)         &   (0.33)         &   (0.20)         &   (0.24)         &   (0.27)         &   (0.30)         &   (0.20)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     0.05         &     0.43\sym{***}&     0.07         &     0.01         &     0.19         &     0.07         &    -0.01         &     0.01         \\
                &   (0.13)         &   (0.10)         &   (0.14)         &   (0.09)         &   (0.13)         &   (0.10)         &   (0.15)         &   (0.13)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Original Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&  298,414         &  163,695         &  224,136         &   95,703         &  154,349         &   49,874         &  112,788         &   30,759         \\
\specialcell{\scriptsize \(R^2\)}&    0.056         &    0.599         &    0.094         &    0.662         &    0.113         &    0.701         &    0.124         &    0.712         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    19.57         &    20.00         &    19.44         &    20.23         &    19.18         &    20.32         &    18.79         &    19.93         \\


==> table/table_ba_1.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize License: Series 65/66 (\%)}}                      \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&    43.37\sym{***}&    32.00\sym{***}&    18.98\sym{***}&    19.67\sym{***}&    21.92\sym{***}\\
                &   (3.28)         &   (2.72)         &   (2.07)         &   (2.16)         &   (2.42)         \\
\addlinespace
\specialcell{\scriptsize Top Adviser $\times$ After}&     5.82\sym{***}&     1.03         &    -5.06\sym{**} &    -4.12\sym{**} &    -6.11\sym{***}\\
                &   (1.92)         &   (1.88)         &   (2.09)         &   (1.98)         &   (1.73)         \\
\addlinespace
\specialcell{\scriptsize Series 63}&                  &   -22.93\sym{***}&   -17.13\sym{***}&                  &                  \\
                &                  &   (1.89)         &   (1.05)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Series 7}&                  &    44.43\sym{***}&    32.79\sym{***}&                  &                  \\
                &                  &   (1.85)         &   (1.16)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Series 6}&                  &    10.79\sym{***}&    -0.23         &                  &                  \\
                &                  &   (1.36)         &   (0.62)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Series 24}&                  &    -9.95\sym{***}&    -1.36\sym{**} &                  &                  \\
                &                  &   (2.12)         &   (0.63)         &                  &                  \\
\addlinespace
\specialcell{\scriptsize Experience}&                  &     0.62\sym{***}&     0.48\sym{***}&     0.84\sym{***}&                  \\
                &                  &   (0.15)         &   (0.08)         &   (0.09)         &                  \\
\addlinespace
\specialcell{\scriptsize Experience squared}&                  &    -0.00         &    -0.02\sym{***}&    -0.03\sym{***}&                  \\
                &                  &   (0.00)         &   (0.00)         &   (0.00)         &                  \\
\addlinespace
\specialcell{\scriptsize Tenure}&                  &    -4.04\sym{***}&    -7.27\sym{***}&    -6.13\sym{***}&    -4.67\sym{***}\\
                &                  &   (0.51)         &   (0.54)         &   (0.58)         &   (0.57)         \\
\addlinespace
\specialcell{\scriptsize Female}&                  &     0.02         &    -0.15         &    -0.17\sym{*}  &    -0.28\sym{***}\\
                &                  &   (0.16)         &   (0.10)         &   (0.09)         &   (0.10)         \\
\addlinespace
\specialcell{\scriptsize Number of Other Licenses}&                  &     3.80\sym{***}&     5.23\sym{***}&     4.22\sym{***}&     3.64\sym{***}\\
                &                  &   (0.68)         &   (0.29)         &   (0.31)         &   (0.51)         \\
\addlinespace
\specialcell{\scriptsize Cumulative Number of Switching Firms}&                  &     0.60\sym{**} &     1.53\sym{***}&     1.21\sym{***}&     0.99\sym{***}\\
                &                  &   (0.28)         &   (0.19)         &   (0.17)         &   (0.23)         \\
\addlinespace
\specialcell{\scriptsize Cumulative Number of Migration Across States}&                  &     3.65\sym{***}&     1.90\sym{***}&     1.84\sym{***}&     1.95\sym{***}\\
                &                  &   (0.48)         &   (0.19)         &   (0.17)         &   (0.21)         \\
\midrule
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&12,396,016         &12,396,016         &11,632,150         &10,614,118         &6,987,781         \\
\specialcell{\scriptsize \(R^2\)}&    0.003         &    0.217         &    0.472         &    0.554         &    0.649         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    35.96         &    35.96         &    36.02         &    34.98         &    30.88         \\


==> table/table_ba_2.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Incidence of Customer Disputes (\%)}}             \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&     2.38\sym{***}&     2.02\sym{***}&     1.63\sym{***}&     1.49\sym{***}&     1.50\sym{***}\\
                &   (0.19)         &   (0.16)         &   (0.12)         &   (0.11)         &   (0.14)         \\
\addlinespace
\specialcell{\scriptsize Top Adviser $\times$ After}&    -1.31\sym{***}&    -1.35\sym{***}&    -0.77\sym{***}&    -0.63\sym{***}&    -0.70\sym{***}\\
                &   (0.22)         &   (0.23)         &   (0.15)         &   (0.13)         &   (0.14)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&12,396,016         &12,396,016         &11,632,150         &10,230,894         &6,466,895         \\
\specialcell{\scriptsize \(R^2\)}&    0.000         &    0.003         &    0.079         &    0.151         &    0.274         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.42         &     0.42         &     0.42         &     0.41         &     0.34         \\


==> table/table_ba_2_1.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Incidence of Customer Disputes (\%)}}             \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&     1.30\sym{***}&     1.01\sym{***}&     0.72\sym{***}&     0.60\sym{***}&     0.45\sym{***}\\
                &   (0.09)         &   (0.08)         &   (0.08)         &   (0.08)         &   (0.12)         \\
\addlinespace
\specialcell{\scriptsize Top Adviser $\times$ After}&    -0.32\sym{**} &    -0.40\sym{***}&    -0.00         &     0.10         &     0.27         \\
                &   (0.13)         &   (0.13)         &   (0.12)         &   (0.12)         &   (0.21)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&12,396,016         &12,396,016         &11,632,150         &10,230,894         &6,466,895         \\
\specialcell{\scriptsize \(R^2\)}&    0.000         &    0.003         &    0.085         &    0.158         &    0.286         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.36         &     0.36         &     0.36         &     0.34         &     0.29         \\


==> table/table_ba_2_2.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Incidence of Customer Disputes (\%)}}             \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&     2.38\sym{***}&     2.02\sym{***}&     1.63\sym{***}&     1.49\sym{***}&     1.50\sym{***}\\
                &   (0.19)         &   (0.16)         &   (0.12)         &   (0.11)         &   (0.14)         \\
\addlinespace
\specialcell{\scriptsize Top Adviser $\times$ After}&    -1.31\sym{***}&    -1.35\sym{***}&    -0.77\sym{***}&    -0.63\sym{***}&    -0.70\sym{***}\\
                &   (0.22)         &   (0.23)         &   (0.15)         &   (0.13)         &   (0.14)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&12,396,016         &12,396,016         &11,632,150         &10,230,894         &6,466,895         \\
\specialcell{\scriptsize \(R^2\)}&    0.000         &    0.003         &    0.079         &    0.151         &    0.274         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.42         &     0.42         &     0.42         &     0.41         &     0.34         \\


==> table/table_bp_1.tex <==
          &\multicolumn{1}{c}{\specialcell{\scriptsize Average Adviser}}&\multicolumn{2}{c}{\specialcell{\scriptsize Top Adviser}}\\\cmidrule(lr){2-2}\cmidrule(lr){3-4}
          &\multicolumn{1}{c}{\specialcell{\scriptsize }}&\multicolumn{1}{c}{\specialcell{\scriptsize Before}}&\multicolumn{1}{c}{\specialcell{\scriptsize After}}\\
\midrule
{\specialcell{\scriptsize \bf Original Firm:}}&         &         &         \\
\hline \quad \specialcell{\scriptsize \bf (1) In the Protocol (\%):}&     21.1&     32.6&     80.4\\
\hline \quad \quad {\specialcell{\scriptsize \bf New Firm:}}&         &         &         \\
\hline \quad \quad \specialcell{\scriptsize \bf (1)-1. In the Protocol (\%):}&     62.9&     90.3&     88.9\\
\hline \quad \quad \quad \ {\specialcell{\scriptsize \bf Pre-Protocol:}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ -3 \ \leq \ t \ \leq \ -1 $}&      5.8&      2.8&      0.7\\
\hline \quad \quad \quad \ {\specialcell{\scriptsize \bf Post-Protocol:}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 0 \ \leq \ t \ \leq \ 2 $}&     36.3&     58.7&     46.2\\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 3 \ \leq \ t \ \leq \ 5 $}&     27.4&     30.6&     14.5\\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 6 \ \leq \ t \ \leq \ 8 $}&     18.1&      6.1&     20.7\\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 9 \ \leq \ t $}&     10.7&      0.9&     17.8\\
\hline  \quad \quad \quad \ {\specialcell{\scriptsize \bf Difference in Firm Size (New-Original):}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize Number of Advisers}&   -728.3&    570.7& -1,600.5\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Assets (in millions of dollars)}&-29,124.0&-29,029.9&-75,463.0\\
\quad \quad \quad \quad \specialcell{\scriptsize AUM (in millions of dollars)}& 35,901.3& 94,995.7& 86,184.4\\
\quad \quad \quad \quad \specialcell{\scriptsize Revenue (in millions of dollars)}& -1,539.4& -5,959.3& -3,098.6\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Number of Accounts (in thousands)}&    243.6&    606.2&    488.8\\
\hline \quad \quad  \specialcell{\scriptsize \bf (1)-2. Not In the Protocol (\%):}&     37.1&      9.7&     11.1\\
\hline  \quad \quad \quad \ {\specialcell{\scriptsize \bf Difference in Firm Size (New-Original):}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize Number of Advisers}&-11,134.5&-11,852.3&-11,321.0\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Assets (in millions of dollars)}&-74,748.9&-78,309.3&-68,296.2\\
\quad \quad \quad \quad \specialcell{\scriptsize AUM (in millions of dollars)}&-79,283.7&-72,789.6&-44,217.6\\
\quad \quad \quad \quad \specialcell{\scriptsize Revenue (in millions of dollars)}& -3,036.1&    -27.7& -3,413.2\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Number of Accounts (in thousands)}&   -432.6&   -369.7&   -308.6\\
\hline {\specialcell{\scriptsize \bf Original Firm:}}&         &         &         \\
\hline \quad \specialcell{\scriptsize \bf (2) Not In the Protocol (\%):}&     78.9&     67.4&     19.6\\
\hline \quad \quad {\specialcell{\scriptsize \bf New Firm:}}&         &         &         \\
\hline \quad \quad \specialcell{\scriptsize \bf (2)-1. In the Protocol (\%):}&     32.7&     68.8&     86.6\\
\hline \quad \quad \quad \ {\specialcell{\scriptsize \bf Pre-Protocol:}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ -3 \ \leq \ t \ \leq \ -1 $}&     32.8&     38.8&      5.7\\
\hline \quad \quad \quad \ {\specialcell{\scriptsize \bf Post-Protocol:}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 0 \ \leq \ t \ \leq \ 2 $}&     23.4&     30.6&     28.6\\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 3 \ \leq \ t \ \leq \ 5 $}&     17.0&     14.0&     18.9\\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 6 \ \leq \ t \ \leq \ 8 $}&     11.2&      6.4&     18.3\\
\quad \quad \quad \quad \specialcell{\scriptsize $ \ 9 \ \leq \ t $}&      4.1&      0.6&     21.1\\
\hline  \quad \quad \quad \ {\specialcell{\scriptsize \bf Difference in Firm Size (New-Original):}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize Number of Advisers}&  6,856.8&  8,161.7&  8,465.1\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Assets (in millions of dollars)}& 33,592.7& 25,747.5&-40,793.5\\
\quad \quad \quad \quad \specialcell{\scriptsize AUM (in millions of dollars)}& 49,248.0& 50,751.5& 80,339.0\\
\quad \quad \quad \quad \specialcell{\scriptsize Revenue (in millions of dollars)}&  1,308.0&   -248.3&   -940.5\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Number of Accounts (in thousands)}&    249.7&    275.9&    376.0\\
\hline \quad \quad  \specialcell{\scriptsize \bf (1)-2. Not In the Protocol (\%):}&     67.3&     31.2&     13.4\\
\hline  \quad \quad \quad \ {\specialcell{\scriptsize \bf Difference in Firm Size (New-Original):}}&         &         &         \\
\quad \quad \quad \quad \specialcell{\scriptsize Number of Advisers}&   -589.4&   -314.2&    199.2\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Assets (in millions of dollars)}& -6,671.3& -8,672.3& -4,319.5\\
\quad \quad \quad \quad \specialcell{\scriptsize AUM (in millions of dollars)}& -4,273.1&-12,856.8& -9,820.3\\
\quad \quad \quad \quad \specialcell{\scriptsize Revenue (in millions of dollars)}&    -81.3&    -55.1&     -5.2\\
\quad \quad \quad \quad \specialcell{\scriptsize Total Number of Accounts (in thousands)}&    -22.4&    -32.5&    -51.0\\
\midrule
Observations&  999,292&    1,833&    1,032\\


==> table/table_bp_2.tex <==
                &\multicolumn{3}{c}{\specialcell{\scriptsize Pre-Protocol: $ -3 \leq x \leq -1 $}}&\multicolumn{3}{c}{\specialcell{\scriptsize Post-Protocol: $ 0 \leq x \leq 2 $}}&\multicolumn{3}{c}{\specialcell{\scriptsize Post-Protocol: $ 3 \leq x \leq 5 $}}&\multicolumn{3}{c}{\specialcell{\scriptsize Post-Protocol: $ 6 \leq x \leq 8 $}}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         &\multicolumn{1}{c}{(9)}         &\multicolumn{1}{c}{(10)}         &\multicolumn{1}{c}{(11)}         &\multicolumn{1}{c}{(12)}         \\
\midrule
\specialcell{\scriptsize Top Adviser}&     0.08\sym{**} &     0.04\sym{*}  &     0.02         &     0.14\sym{***}&     0.07\sym{***}&     0.05\sym{***}&     0.04\sym{*}  &     0.03\sym{***}&     0.01         &    -0.03\sym{**} &     0.01         &     0.00         \\
                &   (0.04)         &   (0.02)         &   (0.01)         &   (0.04)         &   (0.01)         &   (0.01)         &   (0.02)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.00)         \\
\addlinespace
\specialcell{\scriptsize Protocol}&    -0.08\sym{***}&    -0.04\sym{***}&              &     0.12\sym{**} &     0.03\sym{**} &              &     0.10\sym{***}&     0.05\sym{***}&             &     0.06\sym{***}&     0.01         &            \\
                &   (0.02)         &   (0.01)         &             &   (0.06)         &   (0.01)         &             &   (0.03)         &   (0.01)         &             &   (0.02)         &   (0.01)         &             \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ County FE}&                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Year $\times$ County $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&  999,292         &  887,431         &  394,428         &  999,292         &  887,431         &  394,428         &  999,292         &  887,431         &  394,428         &  999,292         &  887,431         &  394,428         \\
\specialcell{\scriptsize \(R^2\)}&    0.019         &    0.449         &    0.670         &    0.061         &    0.452         &    0.640         &    0.041         &    0.425         &    0.668         &    0.029         &    0.403         &    0.681         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     0.09         &     0.09         &     0.13         &     0.11         &     0.10         &     0.10         &     0.08         &     0.07         &     0.06         &     0.05         &     0.05         &     0.04         \\


==> table/table_c_1_1.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     0.42\sym{**} &     0.60\sym{***}&     0.87\sym{***}&     0.81\sym{***}&     1.18\sym{***}&     0.97\sym{***}&     1.24\sym{***}&     0.96\sym{***}\\
                &   (0.18)         &   (0.11)         &   (0.13)         &   (0.10)         &   (0.11)         &   (0.11)         &   (0.11)         &   (0.11)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     1.02\sym{***}&     0.28\sym{***}&     0.88\sym{***}&    -0.03         &     0.82\sym{***}&    -0.01         &     0.82\sym{***}&     0.00         \\
                &   (0.13)         &   (0.07)         &   (0.09)         &   (0.04)         &   (0.11)         &   (0.05)         &   (0.15)         &   (0.05)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&3,657,615         &3,351,286         &2,606,353         &2,315,554         &2,035,744         &1,761,522         &1,629,282         &1,375,548         \\
\specialcell{\scriptsize \(R^2\)}&    0.109         &    0.366         &    0.107         &    0.337         &    0.111         &    0.327         &    0.121         &    0.337         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     7.87         &     7.89         &     7.73         &     7.74         &     7.65         &     7.67         &     7.57         &     7.58         \\


==> table/table_c_1_2.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     2.69\sym{***}&     2.40\sym{***}&     2.98\sym{***}&     2.38\sym{***}&     3.09\sym{***}&     2.47\sym{***}&     2.85\sym{***}&     2.27\sym{***}\\
                &   (0.33)         &   (0.34)         &   (0.27)         &   (0.30)         &   (0.29)         &   (0.34)         &   (0.28)         &   (0.31)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&    -0.22         &     0.09         &    -0.29         &     0.02         &    -0.09         &     0.12         &     0.10         &     0.08         \\
                &   (0.48)         &   (0.17)         &   (0.34)         &   (0.10)         &   (0.29)         &   (0.10)         &   (0.29)         &   (0.07)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&2,947,878         &2,692,018         &2,131,971         &1,882,487         &1,667,690         &1,430,944         &1,327,363         &1,107,899         \\
\specialcell{\scriptsize \(R^2\)}&    0.168         &    0.433         &    0.189         &    0.417         &    0.191         &    0.391         &    0.195         &    0.392         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    19.74         &    19.87         &    19.59         &    19.77         &    19.48         &    19.69         &    19.35         &    19.58         \\


==> table/table_c_2_1.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     0.55\sym{***}&     0.60\sym{***}&     1.09\sym{***}&     0.46\sym{***}&     1.24\sym{***}&     0.45\sym{***}&     1.19\sym{***}&     0.32\sym{***}\\
                &   (0.18)         &   (0.15)         &   (0.11)         &   (0.09)         &   (0.10)         &   (0.09)         &   (0.22)         &   (0.08)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     1.00\sym{***}&     0.35\sym{***}&     0.89\sym{***}&    -0.01         &     0.88\sym{***}&     0.01         &     0.66\sym{***}&     0.08\sym{**} \\
                &   (0.05)         &   (0.04)         &   (0.05)         &   (0.05)         &   (0.08)         &   (0.04)         &   (0.10)         &   (0.04)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Original Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&  348,579         &  194,079         &  261,402         &  113,945         &  182,486         &   61,069         &  134,185         &   38,527         \\
\specialcell{\scriptsize \(R^2\)}&    0.090         &    0.525         &    0.088         &    0.585         &    0.097         &    0.629         &    0.099         &    0.645         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     7.45         &     7.61         &     7.26         &     7.55         &     7.14         &     7.63         &     6.98         &     7.53         \\


==> table/table_c_2_2.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize $0  \leq x \leq  4$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $5  \leq x \leq  9$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $10 \leq x \leq 14$}}&\multicolumn{2}{c}{\specialcell{\scriptsize $15 \leq x \leq 19$}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
\specialcell{\scriptsize Top Adviser (Before Being Ranked)}&     2.52\sym{***}&     1.57\sym{***}&     3.23\sym{***}&     0.92\sym{***}&     3.04\sym{***}&     1.01\sym{***}&     2.64\sym{***}&     0.59\sym{***}\\
                &   (0.39)         &   (0.28)         &   (0.33)         &   (0.20)         &   (0.24)         &   (0.27)         &   (0.30)         &   (0.20)         \\
\addlinespace
\specialcell{\scriptsize Career Start as Investment Adviser}&     0.05         &     0.43\sym{***}&     0.07         &     0.01         &     0.19         &     0.07         &    -0.01         &     0.01         \\
                &   (0.13)         &   (0.10)         &   (0.14)         &   (0.09)         &   (0.13)         &   (0.10)         &   (0.15)         &   (0.13)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Original Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&  298,414         &  163,695         &  224,136         &   95,703         &  154,349         &   49,874         &  112,788         &   30,759         \\
\specialcell{\scriptsize \(R^2\)}&    0.056         &    0.599         &    0.094         &    0.662         &    0.113         &    0.701         &    0.124         &    0.712         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    19.57         &    20.00         &    19.44         &    20.23         &    19.18         &    20.32         &    18.79         &    19.93         \\


==> table/table_jj_1.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Log(Number of Advisers)}}                         &\multicolumn{5}{c}{\specialcell{\scriptsize Log(Total Assets) (in millions of US dollars)}}   \\\cmidrule(lr){2-6}\cmidrule(lr){7-11}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         &\multicolumn{1}{c}{(9)}         &\multicolumn{1}{c}{(10)}         \\
\midrule
\ \specialcell{\scriptsize Top Adviser}&     1.48\sym{***}&     1.15\sym{***}&     0.55\sym{***}&     0.48\sym{***}&     0.43\sym{***}&     3.89\sym{***}&     3.07\sym{***}&     1.19\sym{***}&     1.13\sym{***}&     0.92\sym{***}\\
                &   (0.13)         &   (0.08)         &   (0.06)         &   (0.04)         &   (0.06)         &   (0.31)         &   (0.24)         &   (0.12)         &   (0.13)         &   (0.15)         \\
\addlinespace
\ \specialcell{\scriptsize Top Adviser $\times$ After}&    -0.11         &    -0.15         &    -0.34\sym{***}&    -0.33\sym{***}&    -0.38\sym{***}&    -1.13\sym{***}&    -0.79         &    -0.50\sym{**} &    -0.59\sym{**} &    -0.64\sym{***}\\
                &   (0.21)         &   (0.22)         &   (0.10)         &   (0.09)         &   (0.09)         &   (0.42)         &   (0.49)         &   (0.22)         &   (0.25)         &   (0.24)         \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    -0.59\sym{***}&    -0.59\sym{***}&    -0.46\sym{***}&    -0.40\sym{***}&    -0.30\sym{***}&    -1.44\sym{***}&    -1.40\sym{***}&    -0.92\sym{***}&    -0.85\sym{***}&    -0.74\sym{***}\\
                &   (0.07)         &   (0.05)         &   (0.03)         &   (0.03)         &   (0.03)         &   (0.17)         &   (0.12)         &   (0.06)         &   (0.07)         &   (0.07)         \\
\addlinespace
\ \specialcell{\scriptsize Top Adviser $\times$ Disclosure}&     0.79\sym{***}&     1.01\sym{***}&     0.44\sym{**} &     0.37\sym{*}  &     0.09         &     1.47\sym{***}&     1.36\sym{***}&     1.09\sym{***}&     1.09\sym{***}&     1.30\sym{***}\\
                &   (0.23)         &   (0.24)         &   (0.21)         &   (0.21)         &   (0.29)         &   (0.43)         &   (0.45)         &   (0.34)         &   (0.33)         &   (0.38)         \\
\addlinespace
\ \specialcell{\scriptsize Top Adviser  $\times$ After $\times$ Disclosure}&    -1.05\sym{**} &    -1.24\sym{***}&    -0.86\sym{**} &    -0.84\sym{*}  &    -0.24         &    -0.81         &    -0.74         &    -0.94\sym{*}  &    -1.59\sym{**} &    -0.80         \\
                &   (0.41)         &   (0.41)         &   (0.39)         &   (0.45)         &   (0.47)         &   (0.78)         &   (0.76)         &   (0.55)         &   (0.76)         &   (1.25)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize (Original) Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  &                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  &                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         &                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&1,103,210         &1,103,210         &  984,168         &  792,992         &  441,240         &  935,483         &  935,483         &  827,672         &  661,543         &  365,359         \\
\specialcell{\scriptsize \(R^2\)}&    0.002         &    0.110         &    0.500         &    0.546         &    0.584         &    0.004         &    0.092         &    0.538         &    0.591         &    0.649         \\
\specialcell{\scriptsize Mean of Dependent Variable}&     7.23         &     7.23         &     7.29         &     7.39         &     7.62         &    19.23         &    19.23         &    19.40         &    19.66         &    20.13         \\


==> table/table_js_1.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\ \specialcell{\scriptsize Top Adviser}&    -8.25\sym{***}&    -6.31\sym{***}&    -2.70\sym{***}&    -3.08\sym{***}&    -3.09\sym{***}\\
                &   (1.49)         &   (0.81)         &   (0.47)         &   (0.44)         &   (0.58)         \\
\addlinespace
\ \specialcell{\scriptsize Top Adviser $\times$ After}&    -0.42         &     0.68         &    -1.12\sym{**} &    -0.17         &     0.19         \\
                &   (1.22)         &   (1.82)         &   (0.57)         &   (0.48)         &   (0.63)         \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    13.61\sym{***}&    14.21\sym{***}&     9.29\sym{***}&     9.80\sym{***}&    11.81\sym{***}\\
                &   (0.78)         &   (0.64)         &   (0.43)         &   (0.52)         &   (0.71)         \\
\addlinespace
\ \specialcell{\scriptsize Top Adviser $\times$ Disclosure}&    -9.55\sym{***}&    -9.96\sym{***}&    -8.87\sym{***}&    -9.11\sym{***}&    -9.48\sym{***}\\
                &   (1.94)         &   (1.96)         &   (1.08)         &   (1.06)         &   (1.85)         \\
\addlinespace
\ \specialcell{\scriptsize Top Adviser $\times$ After  $\times$ Disclosure}&     9.94\sym{***}&     9.14\sym{***}&     7.95\sym{***}&     8.09\sym{***}&     9.34\sym{***}\\
                &   (2.47)         &   (2.62)         &   (2.01)         &   (1.73)         &   (2.01)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&11,750,331         &11,750,331         &11,030,563         &9,694,596         &6,149,623         \\
\specialcell{\scriptsize \(R^2\)}&    0.001         &    0.010         &    0.286         &    0.340         &    0.426         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    15.99         &    15.99         &    16.25         &    16.38         &    17.02         \\


==> table/table_ss_1.tex <==
          &\multicolumn{2}{c}{\specialcell{\scriptsize Average Adviser}}&\multicolumn{2}{c}{\specialcell{\scriptsize Top Adviser}}&\multicolumn{1}{c}{\specialcell{\scriptsize Difference}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}
          &     Mean&Std. Dev.&     Mean&Std. Dev.&     Mean         \\
\midrule
{\specialcell{\scriptsize \bf Employment History and Status:}}&         &         &         &         &                  \\
\ \specialcell{\scriptsize Experience (years)}&     11.5&      9.5&     20.9&      9.6&     -9.4\sym{***}\\
\ \specialcell{\scriptsize Tenure (years)}&      5.6&      6.3&     10.4&      9.3&     -4.8\sym{***}\\
\ \specialcell{\scriptsize Currently Registered (in 2018)}&     63.2&     48.2&     91.2&     28.3&    -28.1\sym{***}\\
\hline {\specialcell{\scriptsize \bf Job Transitions (\%):}}&         &         &         &         &                  \\
\hline \ \specialcell{\scriptsize (1) Remain at a Firm}&     84.0&     36.7&     92.3&     26.6&     -8.3\sym{***}\\
\quad \quad {\specialcell{\scriptsize \bf Firm Size:}}&         &         &         &         &                  \\
\quad \quad \ \specialcell{\scriptsize Number of Advisers}&  7,821.1&  9,179.7& 17,063.8& 11,080.7& -9,281.0\sym{***}\\
\quad \quad \ \specialcell{\scriptsize Total Assets (in millions of US dollars)}& 37,653.4& 87,540.1& 99,306.8&105,820.4&-61,894.2\sym{***}\\
\ \specialcell{\scriptsize (2) Leave a Firm}&     16.0&     36.7&      7.7&     26.6&      8.3\sym{***}\\
\hline \quad {\specialcell{\scriptsize \bf Conditional on Leaving a Firm:}}&         &         &         &         &                  \\
\hline \quad \ \specialcell{\scriptsize New Employment (\%)}&     58.7&     49.2&     92.1&     27.0&    -33.4\sym{***}\\
\quad \quad {\specialcell{\scriptsize \bf Original Firm Size:}}&         &         &         &         &                  \\
\quad \quad \ \specialcell{\scriptsize Number of Advisers}&  6,171.3&  8,418.9& 12,420.8& 10,841.8& -6,267.3\sym{***}\\
\quad \quad \ \specialcell{\scriptsize Total Assets (in millions of US dollars)}& 42,572.3& 92,934.9&142,462.5&127,705.5&-100,166.0\sym{***}\\
\quad \quad {\specialcell{\scriptsize \bf New Firm Size:}}&         &         &         &         &                  \\
\quad \quad \ \specialcell{\scriptsize Number of Advisers}&  6,634.2&  9,305.8& 14,359.1& 10,968.6& -7,746.7\sym{***}\\
\quad \quad \ \specialcell{\scriptsize Total Assets (in millions of US dollars)}& 34,374.1& 83,991.3& 88,143.6&111,335.8&-53,899.4\sym{***}\\
\quad \quad {\specialcell{\scriptsize \bf Migration Across (\%):}}&         &         &         &         &                  \\
\quad \quad \quad \specialcell{\scriptsize States}&     41.5&     49.3&     33.9&     47.4&      7.6\sym{***}\\
\quad \quad \quad \specialcell{\scriptsize Commuting Zones}&     48.0&     50.0&     37.0&     48.3&     11.0\sym{***}\\
\quad \quad \quad \specialcell{\scriptsize Counties}&     56.2&     49.6&     41.0&     49.2&     15.2\sym{***}\\
\hline {\specialcell{\scriptsize \bf Licenses/Qualifications (\%):}}&         &         &         &         &                  \\
\ \specialcell{\scriptsize Series 63 (General Securities Agent)}&     73.6&     44.1&     91.4&     28.1&    -17.8\sym{***}\\
\ \specialcell{\scriptsize Series 7 (General Securities Representative)}&     64.5&     47.8&     93.2&     25.2&    -28.8\sym{***}\\
\ \specialcell{\scriptsize Series 6 (Insurance and Annuities)}&     37.9&     48.5&      8.1&     27.3&     29.8\sym{***}\\
\ \specialcell{\scriptsize Series 65/66 (Investment Adviser)}&     35.2&     47.8&     81.5&     38.9&    -46.4\sym{***}\\
\ \specialcell{\scriptsize Series 24 (Principal/Supervisory Management)}&     13.4&     34.1&     12.7&     33.2&      0.7\sym{***}\\
\hline \ \specialcell{\scriptsize Total Number of Licenses}&      2.7&      1.4&      3.9&      1.3&     -1.2\sym{***}\\
\midrule
Observations&12,898,909&         &   46,553&         &12,898,909         \\


==> table/table_ss_2.tex <==
                &\multicolumn{2}{c}{\specialcell{\scriptsize Average Adviser}}&\multicolumn{2}{c}{\specialcell{\scriptsize Top Adviser}}&\multicolumn{1}{c}{\specialcell{\scriptsize Difference}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}
                &     Mean& Std.Dev.&     Mean& Std.Dev.&     Mean         \\
\midrule
{\specialcell{\scriptsize \bf Customer Disputes (\%):}}&         &         &         &         &                  \\
\ \specialcell{\scriptsize Customer Disputes - Settled}&     0.32&     5.65&     1.37&    11.64&    -1.06\sym{***}\\
\ \specialcell{\scriptsize Customer Disputes - Award/Judgment}&     0.03&     1.73&     0.15&     3.87&    -0.12\sym{***}\\
\hline \ \specialcell{\scriptsize Any Customer Dispute with Settlement}&     0.35&     5.89&     1.51&    12.20&    -1.17\sym{***}\\
\hline \ \specialcell{\scriptsize Customer Disputes - Denied}&     0.32&     5.62&     1.66&    12.77&    -1.35\sym{***}\\
\ \specialcell{\scriptsize Customer Disputes - Closed-No Action}&     0.08&     2.87&     0.49&     7.01&    -0.41\sym{***}\\
\ \specialcell{\scriptsize Customer Disputes - Dismissed}&     0.00&     0.34&     0.01&     1.04&    -0.01\sym{*}  \\
\ \specialcell{\scriptsize Customer Disputes - Withdrawn}&     0.02&     1.25&     0.11&     3.24&    -0.09\sym{***}\\
\hline \ \specialcell{\scriptsize Any Customer Disputes without Settlement}&     0.41&     6.39&     2.23&    14.76&    -1.83\sym{***}\\
\hline \ \specialcell{\scriptsize Customer Disputes - Pending}&     0.04&     2.00&     0.09&     3.07&    -0.05\sym{***}\\
\hline \ \specialcell{\scriptsize Any Customer Dispute}&     0.77&     8.72&     3.67&    18.80&    -2.91\sym{***}\\
\hline {\specialcell{\scriptsize \bf Disciplinary Actions (\%):}}&         &         &         &         &                  \\
\ \specialcell{\scriptsize Employment Separation After Allegations }&     0.15&     3.90&     0.12&     3.53&     0.03         \\
\ \specialcell{\scriptsize Regulatory - Final}&     0.12&     3.42&     0.16&     3.96&    -0.04\sym{*}  \\
\hline \ \specialcell{\scriptsize Any Disciplinary Action}&     0.26&     5.07&     0.26&     5.09&    -0.00         \\
\hline {\specialcell{\scriptsize \bf Other Disclosure Events (\%):}}&         &         &         &         &                  \\
\ \specialcell{\scriptsize Criminal Disposition - Final}&     0.03&     1.73&     0.01&     1.14&     0.02\sym{**} \\
\ \specialcell{\scriptsize Civil - Final}&     0.00&     0.62&     0.00&     0.46&     0.00         \\
\ \specialcell{\scriptsize Financial - Final}&     0.27&     5.16&     0.02&     1.47&     0.25\sym{***}\\
\ \specialcell{\scriptsize Judgment/Lien}&     0.22&     4.64&     0.01&     1.04&     0.21\sym{***}\\
\ \specialcell{\scriptsize Civil Bond}&     0.00&     0.33&     0.00&     0.00&     0.00\sym{***}\\
\ \specialcell{\scriptsize Criminal - Pending}&     0.01&     0.79&     0.00&     0.46&     0.00         \\
\ \specialcell{\scriptsize Civil - Pending}&     0.00&     0.26&     0.00&     0.00&     0.00\sym{***}\\
\ \specialcell{\scriptsize Financial - Pending}&     0.03&     1.69&     0.00&     0.46&     0.03\sym{***}\\
\ \specialcell{\scriptsize Regulatory - Pending}&     0.00&     0.44&     0.00&     0.00&     0.00\sym{***}\\
\ \specialcell{\scriptsize Criminal - On Appeal}&     0.00&     0.11&     0.00&     0.00&     0.00\sym{***}\\
\ \specialcell{\scriptsize Civil - On Appeal}&     0.00&     0.11&     0.00&     0.00&     0.00\sym{***}\\
\ \specialcell{\scriptsize Regulatory - On Appeal}&     0.00&     0.23&     0.00&     0.00&     0.00\sym{***}\\
\ \specialcell{\scriptsize Investigation}&     0.00&     0.68&     0.00&     0.66&     0.00         \\
\hline {\specialcell{\scriptsize \bf All Disclosure Events (\%):}}&         &         &         &         &                  \\
\ \specialcell{\scriptsize Any Disclosure Event}&     1.52&    12.22&     3.93&    19.43&    -2.42\sym{***}\\
\midrule
Observations    &12,898,909&         &   46,553&         &12,898,909         \\


==> table_tex/t_13.tex <==
%---------------------------------------------------------------------------
% Protocol for Broker Recruting
% 2008--2018
% Top Adviser
%----------------------------------------------------------------
% Three Time-Phases After Firm in the Protocol:
%----------------------------------------------------------------
\begin{sidewaystable}[hbtp!]
%\begin{table}[htbp!]
\centering
%	\tiny
%	\setlength{\tabcolsep}{3pt}
\scriptsize 
\setlength{\tabcolsep}{3pt}
%	\footnotesize 
%	\setlength{\tabcolsep}{3pt}
%----------------------------------------------------------------
\caption{Sorting Dynamics After Firms Join the Protocol for Broker Recruting}
\label{table: bp 2}
%----------------------------------------------------------------
\begin{threeparttable}
%----------------------------------------------------------------
% Before & After:

% 3 Periods Combined:

%\estauto{esttab_broker_protocol_all_post_periods_year_condition_2_top_adviser_before_after_2000_2018.tex}{12}{c}	
%\estauto{esttab_broker_protocol_all_post_periods_year_condition_2_top_adviser_before_after_2000_2018_omit.tex}{12}{c}	

% 4 time-phases:
%\estauto{esttab_broker_protocol_four_post_periods_year_condition_2_top_adviser_before_after_2000_2018.tex}{12}{c}
%\estauto{esttab_broker_protocol_four_post_periods_year_condition_2_top_adviser_before_after_2000_2018_omit.tex}{12}{c}

%	Two Fixed Effects:
%\estauto{esttab_broker_protocol_two_fixed_effects_year_condition_2_top_adviser_before_after_2000_2018_omit.tex}{12}{c}
%----------------------------------------------------------------
% Before Only:
%----------------------------------------------------------------

% 4 time-phases:
%\estauto{esttab_broker_protocol_four_post_periods_year_condition_2_top_adviser_before_only_2000_2018.tex}{12}{c}
%\estauto{esttab_broker_protocol_four_post_periods_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}

% Two Fixed Effects:
%\estauto{esttab_broker_protocol_two_fixed_effects_three_year_windows_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_two_fixed_effects_2_three_year_windows_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}

% 0-3; 4-5; 6-8
%\estauto{esttab_broker_protocol_two_fixed_effects_2_3_year_windows_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_two_fixed_effects_2_2_3_year_windows_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}

% Pre- & Post Protocol:

%\estauto{esttab_broker_protocol_two_fixed_effects_pre_post_period_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_two_fixed_effects_2_pre_post_period_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}
%----------------------------------------------------------------
%\estauto{esttab_broker_protocol_pre_post_period_year_condition_2_top_adviser_before_only_2000_2018_omit.tex}{12}{c}

% 4 years intervals
%\estauto{esttab_broker_protocol_pre_post_period_year_condition_1_top_adviser_1_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_period_year_condition_1_top_adviser_2_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_period_year_condition_2_top_adviser_1_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_period_year_condition_2_top_adviser_2_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_period_year_condition_3_top_adviser_1_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_period_year_condition_3_top_adviser_2_before_only_2000_2018_omit.tex}{12}{c}

% 3 years intervals
%\estauto{esttab_broker_protocol_pre_2_post_period_year_condition_2_top_adviser_1_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_2_post_period_year_condition_2_top_adviser_2_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_2_post_period_year_condition_3_top_adviser_1_before_only_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_2_post_period_year_condition_3_top_adviser_2_before_only_2000_2018_omit.tex}{12}{c}
%----------------------------------------------------------------

%\begin{center}
%	{\bf 2001--2016}
%\end{center}
%----------------------------------------------------------------

%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_1_top_adviser_1_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_1_top_adviser_2_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_2_top_adviser_1_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_2_top_adviser_2_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_3_top_adviser_1_2000_2018_omit.tex}{12}{c}
%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_3_top_adviser_2_2000_2018_omit.tex}{12}{c}
%----------------------------------------------------------------
% Shorter Intervals:
%\estauto{esttab_broker_protocol_shorter_pre_post_period_year_condition_1_top_adviser_1_2000_2018_omit.tex}{20}{c}
%\estauto{esttab_broker_protocol_shorter_pre_post_period_year_condition_1_top_adviser_2_2000_2018_omit.tex}{20}{c}
%\estauto{esttab_broker_protocol_shorter_pre_post_period_year_condition_2_top_adviser_1_2000_2018_omit.tex}{20}{c}
%\estauto{esttab_broker_protocol_shorter_pre_post_period_year_condition_2_top_adviser_2_2000_2018_omit.tex}{20}{c}
%\estauto{esttab_broker_protocol_shorter_pre_post_period_year_condition_3_top_adviser_1_2000_2018_omit.tex}{20}{c}
%\estauto{esttab_broker_protocol_shorter_pre_post_period_year_condition_3_top_adviser_2_2000_2018_omit.tex}{20}{c}
%----------------------------------------------------------------
% without Interaction Term:
%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_1_top_adviser_1_2000_2018_without_interaction_omit.tex}{20}{c}
%\estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_1_top_adviser_2_2000_2018_without_interaction_omit.tex}{20}{c}
% \estauto{esttab_broker_protocol_pre_post_3_year_windows_year_condition_1_top_adviser_2_2000_2018_without_interaction_omit_fixed.tex}{20}{c}
\estauto{table/table_bp_2.tex}{20}{c}
%----------------------------------------------------------------
\Fignote{%
Observations are based on adviser-year panel data over the period 2001-2016.
%	Conditional on that an adviser worked for a firm in the year $t$ and switches to a new firm by the end of the next year $t+1$, 
%	the dependent variable is a dummy that indicates whether an adviser move to a firm in the protocol at $t+1$.
The dependent variable is a dummy that indicates whether an adviser move to a firm in the protocol at $t+1$,
conditional on that 
the adviser worked for a firm in the previous year $t$ and switched to a new firm by the end of the next year $t+1$.  
Note that the sample does not include observations that advisers exit from the industry over the period.
The variable ``$\text{Protocolo}$" is a dummy for whether the former firm at time $t$ was in the protocol. 
%	The coefficients are in percentage points. 
Standard errors are in brackets and clustered by firms.  \\
\text{* $p < 0.10$, ** $p < 0.05$, *** $p < 0.01$.}
}
%----------------------------------------------------------------
\end{threeparttable}
%\end{table}
\end{sidewaystable}
%---------------------------------------------------------------------------
